Partial Regularization of First-Order Resolution Proofs

Resolution and superposition are common techniques which have seen widespread use with propositional and first-order logic in modern theorem provers. In these cases, resolution proof production is a key feature of such tools; however, the proofs that they produce are not necessarily as concise as possible. For propositional resolution proofs, there are a wide variety of proof compression techniques. There are fewer techniques for compressing first-order resolution proofs generated by automated theorem provers. This paper describes an approach to compressing first-order logic proofs based on lifting proof compression ideas used in propositional logic to first-order logic. One method for propositional proof compression is partial regularization, which removes an inference $\eta$ when it is redundant in the sense that its pivot literal already occurs as the pivot of another inference in every path from $\eta$ to the root of the proof. This paper describes the generalization of the partial-regularization algorithm RecyclePivotsWithIntersection [10] from propositional logic to first-order logic. The generalized algorithm performs partial regularization of resolution proofs containing resolution and factoring inferences with unification. An empirical evaluation of the generalized algorithm and its combinations with the previously lifted GreedyLinearFirstOrderLowerUnits algorithm [12] is also presented

==> FOSubExample.tex <==
Recall example \ref{ex:ambig}. In order to avoid this, we introduce a proof rule that applies a substitution. So that we would get the following proof

\begin{tiny}
\begin{prooftree}
\def\e{\mbox{\ $\vdash$\ }}
\AxiomC{$\eta_1$: $p(U),r(U~V),r(V~U),q(V)$\e}
\UnaryInfC{$\eta_2$: $p(c),r(c~V),r(V~c),q(V)$\e}
\AxiomC{$\eta_3$: \e$r(X~c)$}
\BinaryInfC{$\eta_4$: $p(c),r(c~X),q(X)$\e}
\AxiomC{$\eta_5$: \e$r(W~V)$}
\BinaryInfC{$\eta_6$: $p(c),q(V)$\e}
\AxiomC{$\eta_7$: $p(Z)$\e$q(d)$}
\BinaryInfC{$\eta_8$: $p(c),p(Z)$\e}
\UnaryInfC{$\eta_9$: $p(c)$\e}
\AxiomC{$\eta_{10}$: \e$p(c)$}
\BinaryInfC{$\psi$: $\bot$}
\end{prooftree}
\end{tiny}

Now $r(V, c)$ appears in the first left resolvent, which was the left aux formula in the original proof. Thus, the implementation can find that formula, and choose it in order to resolve the ambiguous resolution, instead of guessing a formula from the left resolvent that unifies with the right resolvent, which might go wrong.\\

TODO: Explain where the sub came from.\\

TODO: define the rule formally here?\\

TODO: describe when the rule is invoked in the implementation\\

==> olddefn.tex <==
\begin{definition}[First-Order Resolution Proof] 
\label{def:proof} \hfill \\
A directed acyclic graph $\langle V, E, \clause \rangle$, where $V$ is a set of nodes and $E$ is a
set of edges labeled by literals and substitutions (i.e. $E \subset V \times 2^{\mathcal{L}} \times \mathcal{S} \times V$, where $\mathcal{L}$ is the set of all literals and $\mathcal{S}$ is the set of all substitutions, and $\n_1
\xrightarrow[\sigma]{\ell} \n_2$ denotes an edge from node $\n_1$ to node $\n_2$ labeled by the literal $\ell$ and the substitution $\sigma$), is a
proof of a clause $\clause$ iff it is inductively constructible according to the following cases:
%
\begin{itemize}
  \item \textbf{Axiom:} If $\Gamma$ is a clause, $\axiom{\Gamma}$ denotes some proof $\langle \{ \n \}, \varnothing,
    \Gamma \rangle$, where $\n$ is a new (axiom) node.
  \item \textbf{Resolution\footnote{This is referred to as ``binary resolution'' elsewhere, with the understanding that ``binary'' refers to the number of resolved literals, rather than the number of premises of the inference rule.}:} If $\psi_L$ is a proof $\langle V_L, E_L, \clause_L \rangle$ with $\ell_L \in \clause_L$ and
    $\psi_R$ is a proof $\langle V_R, E_R, \clause_R \rangle$ with $\ell_R \in \clause_R$, and 
    $\sigma_L$ and $\sigma_R$ are substitutions such that
    $\ell_L \sigma_L = \dual{\ell_R} \sigma_R$ %and
    %$\freevar{\left( \clause_L \setminus \left\{ \ell_L \right\} \right) \sigma_L} \cap 
     %\freevar{\left( \clause_R
     %               \setminus \left\{ \ell_R \right\} \right) \sigma_R} = \emptyset$, 
    then
    $\psi_L \res{\ell_L}{\sigma_L}{\ell_R}{\sigma_R} \psi_R$ denotes a proof $\langle V, E, \Gamma \rangle$ s.t.
    \begin{align*}
     \hspace{-0.6cm} V &= V_L \cup V_R \cup \{\n \}    \\
      \hspace{-0.6cm} E &= E_L \cup E_R \cup 
                    \left\{ \raiz{\psi_L} \xrightarrow[\sigma_L]{\{\ell_L\} } \n, 
                            \raiz{\psi_R} \xrightarrow[\sigma_R]{\{\ell_R\} } \n \right\}    \\
    \hspace{-0.6cm}  \Gamma &= \left( \clause_L \setminus \left\{ \ell_L \right\} \right) \sigma_L \cup \left( \clause_R
                    \setminus \left\{ \ell_R \right\} \right) \sigma_R
    \end{align*}
    where $\n$ is a new (resolution) node and $\raiz{\varphi}$ denotes the root node of $\varphi$. $\ell_L$ and $\ell_R$ are $\n$'s \emph{resolved literals}, whereas $\ell_L \sigma_L$ and $\ell_R \sigma_R$ are its \emph{instantiated resolved literals}. The \emph{pivot} of $\n$ is the underlying atom of its instantiated resolved literals (i.e. $\abs{\ell_L \sigma_L}$ or, equivalently, $\abs{\ell_R \sigma_R}$).
  \item \textbf{Factoring:}
  %\footnote{This is often called ``Factoring'', but we prefer ``contraction'', because it is essentially the contraction rule of sequent calculus generalized with unification.} 
  If $\psi'$ is a proof $\langle V', E', \clause' \rangle$ and $\sigma$ is a unifier of $\{\ell_1, \ldots \ell_n\}$ with $\{\ell_1, \ldots \ell_n\} \subseteq \clause'$, then $\con{\psi}{\{\ell_1, \ldots \ell_n\}}{\sigma}$ denotes a proof $\langle V, E, \Gamma \rangle$ s.t.
    \begin{align*}
         \hspace{-0.6cm} V &= V' \cup \{\n \} \\
         \hspace{-0.6cm} E &= E' \cup \{ \raiz{\psi'} \xrightarrow[\sigma]{\{\ell_1, \ldots \ell_n\}} \n \} \\
       \hspace{-0.6cm} \Gamma &= (\clause' \setminus \{ \ell_1, \ldots \ell_n \} ) \sigma \cup \{ \ell \}
    \end{align*}
    where $\n$ is a new (factoring) node, $\ell = \ell_k \sigma$ (for any $k \in \{1,\ldots, n\}$) and $\raiz{\varphi}$ denotes the root node of $\varphi$.
  \qed
\end{itemize}
\end{definition}

==> oldlemma.tex <==
\begin{lem}\label{lem:cor}
Let $\eta_1$ be a node and $\rho(\eta_1)$ be a path from $\eta_1$ to the root of the proof. Suppose that $\eta \in \rho(\eta_1)$ is the direct descendant of $\eta_1$ on $\rho(\eta_1)$ such that $\eta_1 \sqsubseteq \mathcal{S}(\eta)$. If $\eta$ is replaced by $\eta_1$ in some proof $\psi$ to obtain $\psi'$, every literal $\ell_s \in \eta_1$ is either used as a pivot below $\eta_1$ in $\psi'$ or is contained in the root clause $\Gamma(\psi')$. \\
\end{lem}

\begin{proof}
For a pair of nodes $\eta_1$, $\eta$ that satisfy the conditions of the lemma, let $\sigma_1$ be the substitution such that $\eta_1\sigma_1 \subseteq \mathcal{S}(\eta)$. Assume that $\eta_1 \xrightarrow[\sigma]{\{\ell_1\} } \eta$ in $\psi$.

We proceed by induction $h(\eta)$, the height of $\eta$ in $\psi$, which is the length of a longest path from the root to $\eta$. For the base case $h(\eta)=0$, when deleting $\eta$, $\eta$ is replaced by $\eta_1$ and by assumption there exists a $\sigma_1$ such that $\Gamma(\eta_1)\sigma_1 \subseteq \mathcal{S}(\eta) = \Gamma(\eta) \implies \Gamma(\eta_1) \sqsubseteq \Gamma(\eta)$. %This concludes the base case; assume the result holds for any node $\eta_I$ with height $h(\eta_I) > 0$ and consider a node $\eta$ at height $h(\eta)=h(\eta_I)+1$.
This concludes the base case; assume the result holds for any node $\eta_I$ with height $h(\eta_I) \le m$ for an arbitrary $m$ and consider a node $\eta$ at height $h(\eta)=m+1$.

For the inductive step, 
consider any path $\rho(\eta')$ from $\eta'$ to the root of the proof, and let $\eta''$ be the node which is resolved against $\eta$ in $\psi$. The deletion of $\eta$ from $\psi$ attempts to replace the resolution $\eta'=\eta \odot \eta''$ with $\eta' = \eta_1 \odot \eta''$.

For each path $\rho(\eta')$, there are two cases: either there exists an $\ell_1''\in \eta_1$ such that $\ell_1''\sigma_1$ can be used as the instantiated resolved literal between $\eta_1$ and $\eta'''$, or no such $\ell_1''$ exists.\\

\noindent
\emph{Case 1:}  $\eta_1 \xrightarrow[\sigma_1''=\sigma_1]{\{\ell_1''\} } \eta'$ and $\eta'' \xrightarrow[\sigma_2'']{\{\ell_2''\} } \eta'$ for some $\ell_1''$, $\ell_2''$, and $\sigma_2''$.

Since all instantiated literals of $\eta_1\sigma_1$ are safe, for each of the remaining literals $\ell_s \sigma_1 \in \Gamma(\eta_1)\sigma_1 \cap \Gamma(\eta')$ such that $\ell_s\neq \ell_1''$, there is a node $\eta_{\ell_s}\in \rho(\eta')$ that uses $\ell_s\sigma_1$ as a resolved literal or $\ell_s\sigma_1$ is contained in the root clause $\Gamma$; i.e. every remaining literal $\ell \in \eta_1$ that is not contained in $\Gamma$ will eventually be used as a resolved literal. The nodes using $\ell_{\eta''}\sigma_2'' \in (\Gamma(\eta'')\sigma_2''\cap\Gamma(\eta'))\setminus (\Gamma(\eta_1)\sigma_1)$ are unchanged, so these literals will still be used as a resolved literal for some node below $\eta'$. 
It remains to be shown that $\ell_1$ is still used as a resolved literal. To see this, recall that clauses are sets and that $\ell_1\sigma_1$ is safe. Therefore the resolution on $\rho(\eta')$ which uses $\ell_1\sigma_1$ as a resolved literal removes all copies\footnote{Note that the desired result can be obtained by inserting a factoring node before performing resolution with $\eta'$ if clauses are defined as multi-sets.} of $\ell_1\sigma_1$. \\


\noindent
\emph{Case 2:} $\sigma_1$ cannot be used as a unifier for literals of $\eta_1$ and $\eta''$; i.e. resolution between $\eta_1$ and $\eta''$ is not possible for any $\ell_1''\in \eta_1$ 
with the instantiated resolved literal $\ell_1''\sigma_1$. In this case, replace $\eta'$ by $\eta_1$; since $\ell_1''\sigma_1'' \notin \Gamma(\eta_1)\sigma_1$, every $\ell_s\sigma_1 \in \Gamma(\eta_1)\sigma_1$ must still be used as a resolved literal below $\eta'$, i.e. $\eta_1\sigma_1 \subseteq \mathcal{S}(\eta') \implies \eta_1 \sqsubseteq \mathcal{S}(\eta')$. Since $h(\eta') < h(\eta)=m+1$, we are done by the induction hypothesis. 


\end{proof}

\begin{proof}[Proof of Theorem \ref{thm:correct}]
Let $\psi$ be a proof with root clause $\Gamma$, and let $\eta_S \in \psi$ be a strongly regularizable node.  Let $\psi' = \psi\setminus \{\eta_S\}$ with root clause $\Gamma'$. To prove the theorem, it suffices to observe that any strongly regularizable node $\eta_S$ satisfies Lemma \ref{lem:cor}'s hypothesis for any $\rho(\eta_1)$.



\begin{figure}[bt]
\begin{centering}
\scalebox{0.8}{
\begin{tikzpicture}
  \tikzstyle{vertex}=[circle,minimum size=10pt,inner sep=0pt]
\tikzset{edge/.style = {->,> = latex'}}

    \node[vertex] (n1) at (-2,1) {$\eta_1$};
    \node[vertex] (n2) at (0,1) {$\eta_2$};
    \node[vertex] (n5) at (1,0.5) {$\eta''$};
    \node[vertex] (n3) at (-1,0.5) {$\eta$};
    \node[vertex] (r) at (0,0) {$\eta'$};

\draw[edge] (r) -- (n5);
\draw[edge] (r) -- (n3);
\draw[edge] (n3) -- (n1);
\draw[edge] (n3) -- (n2);


    \node[vertex] (m1) at (2,1) {$ $};
        \node[vertex] (m2) at (3,1) {$ $};
\draw[edge] (m1)  -- (m2);

    \node[vertex] (ndp) at (6,0.5) {$\eta''$};
    \node[vertex] (n) at (4,0.5) {$\eta_1$};
    \node[vertex] (rp) at (5,0) {$\eta'$};
\draw[edge] (rp) -- (ndp);
\draw[edge] (rp) -- (n);
\end{tikzpicture}
}
\end{centering}
\caption{The a layout of $\eta_1$ and $\eta$ in proofs $\psi$ (left) and $\psi\setminus\{\eta\}$ (right), as used in the proof of Lemma \ref{lem:cor}.}
\label{fig:dagex}
\end{figure}



\end{proof}

==> propRPIex.tex <==
\begin{example}
When applied to the proof $\psi$ shown in Example \ref{Example:Proof}, the algorithm {\RPI} assigns $\{a,c\}$ and $\{a, \neg c\}$ as the safe literals of, respectively, $\eta_5$ and $\eta_8$. The safe literals of $\eta_4$ w.r.t. its children $\eta_5$ and $\eta_8$ are respectively $\{a,c,b\}$ and $\{a, \neg c, b\}$, and hence the safe literals of $\eta_4$ are $\{a,b\}$ (the intersection of $\{a,c,b\}$ and $\{a, \neg c, b\}$). Since the right resolved literal of $\eta_4$ ($a$) belongs to $\eta_4$'s safe literals, $\eta_4$ is correctly detected as a redundant node and hence regularized: $\eta_4$ is replaced by its right parent $\eta_3$. The resulting proof is shown below:

\begin{small}
\begin{prooftree}
\AXC{$ \eta_1: \neg a $}
		\AXC{$ \eta_2: a, c, \neg b $}
						\AXC{$ \eta_3:  a, b $}\RName{$ $}
			\BIC{$ \eta_5: a, c$}	\RName{$ $}
	\BIC{$\eta_6: c$}
		\AXC{$ \eta_3 $}
				\AXC{$ \eta_7: a, \neg c, \neg b $} \RName{$ $}
			\BIC{$ \eta_8: a, \neg c$}	\RName{$ $}
					\AXC{$ \eta_1 $}  \RName{$ $}
				\BIC{$ \eta_9: \neg c$}	\RName{$ $}
		\BIC{$\psi: \bot$}	
\end{prooftree}
\end{small}

%This proof corresponds to the proof term
$$
(\ub{\{\neg a\}}{\eta_1} \tRes (\{a, c, \neg b\} \tRes \ub{\{a, b\}}{\eta_3})) \tRes ((\eta_3 \tRes \{\neg b, \neg c, a\}) \tRes \eta_1)
$$
%
\noindent%
{\RP}, on the other hand, assigns $\emptyset$ as the set of safe literals for $\eta_4$. Therefore, it does not detect that $\eta_4$ is a redundant irregular node, and then $\RP(\varphi) = \varphi$. 
 %
\hfill\QED
\end{example}

\begin{theorem}
\label{Theorem:RPIBetterThanRP}
For any proof $\varphi$, $|\RPI(\varphi)| \leq |\RP(\varphi)|$.
\end{theorem}
\begin{proof}
  For every node $\eta$ in $\varphi$, let $S^{\eta}_{\RPI}$ (resp.,
  $S^{\eta}_{\RP}$) be the set of safe literals for $\eta$ computed by {\RPI} and
  {\RP}. It is easy to see that $S^{\eta}_{\RPI} \supseteq S^{\eta}_{\RP}$ for all
  $\eta$. Therefore, {\RPI} detects and eliminates more redundancies than {\RP}.
%
\hfill\QED
\end{proof}

The better compression of {\RPI} does not come for free, 
as computing an intersection of sets is more costly than assigning the empty set. 
For a node $\eta$ with $k$ children, $k$ sets must be intersected and the size of each set is 
in the worst case in $O(h)$, where $h$ is the length of the shortest path from $\eta$ to a root.

==> sec-FOLU.tex <==


\section{First-Order LowerUnits} \label{sec:FOLU}

The examples shown in the previous section indicate that there are two main challenges that need to be overcome in order to generalize \LowerUnits to the first-order case:
\begin{enumerate}
\item The deletion of a node changes literals. Since substitutions associated with the deleted node are not applied anymore, some literals become more general. Therefore, the reconstruction of the proof during deletion needs to take such changes into account.
\item Whether a unit should be collected for lowering must depend on whether the literals that were resolved with the unit's single literal are unifiable after they are propagated down to the bottom of the proof by the process of unit deletion. Only if this is the case, they can be contracted and the unit can be reintroduced in the bottom of the proof.
\end{enumerate}

\newcommand{\none}{\texttt{none}}

\noindent
Algorithm \ref{algo:fodel} overcomes the first challenge by keeping an additional map from old literals in the input proof to the corresponding more general changed literals in the output proof unders construction. This is done in lines 6 to 7. The correspondence can be computed by proper bookkeeping during deletion (e.g. by having data structures that preserve the positions of literals or by annotating literals with ids). In cases where, due to previous deletions above in the proof, no corresponding literal is available anymore, the special constant $\none$ is used. 

Not only the literals, but also the substitutions must change during deletion. While it would be in principle possible to keep track of such changes as well, it is simpler to search for new substitutions that result in a most general resolved atom. This is why substitutions are omitted in line 12. As a beneficial side-effect, we may obtain more general literals in the root clause of the output proof.


\SetKwFunction{Rec}{delete}
\SetKw{Let}{let}

\newcommand{\dl}[1]{#1^{\dagger}}

\begin{algorithm}[bt]
  \SetAlgoVlined
  \SetAlgoShortEnd
  \KwIn{a proof $\varphi$}
  \KwIn{$D$ a set of subproofs}
  \KwOut{a proof $\varphi'$ obtained by deleting the subproofs in $D$ from $\varphi$}
  \KwData{a map $.'$, initially empty, eventually mapping any $\xi$ to \Del{$\xi$, $D$}}
  \KwData{a map $\dl{.}$, initially empty, eventually mapping literals to changed literals}
  \BlankLine

  \newcommand{\fixL}{\ensuremath{\varphi'_L}}
  \newcommand{\fixR}{\ensuremath{\varphi'_R}}

  \lIf{$\varphi \in D$ or $\raiz{\varphi}$ has no premises}{\Return{$\varphi$}}
  \BlankLine

  \ElseIf{$\varphi = \varphi_L \res{\ell_L}{\sigma_L}{\ell_R}{\sigma_R} \varphi_R$}{
    $\varphi'_L \leftarrow $ \Rec{$\varphi_L$,$D$} \;
    $\varphi'_R \leftarrow $ \Rec{$\varphi_R$,$D$} \;
    \BlankLine

    \For{every $\ell$ in $\Conclusion{\varphi_L}$ or $\Conclusion{\varphi_R}$}{
      $\dl{\ell} \leftarrow$ the literal in $\Conclusion{\varphi'_L}$ or $\Conclusion{\varphi'_R}$ corresponding to $\ell$, otherwise $\none$ \;
    }

    \lIf{$\varphi'_L \in D$}{ 
      \Return{\fixR} 
    }
    \lElseIf{$\varphi'_R \in D$}{ 
      \Return{\fixL}  
    }
    \BlankLine

    \lElseIf{$\dl{\ell_L} = \none$}{ 
      \Return{\fixL} 
    }
    \lElseIf{$\dl{\ell_R} = \none$}{ 
      \Return{\fixR}  
    }
    \BlankLine

    \lElse{ 
      \Return{ \fixL~$\res{\dl{\ell_L}}{}{\dl{\ell_R}}{}$~\fixR}
    }
  }
  \ElseIf{$\varphi = \con{\varphi_c}{ \{\ell_1,\ldots,\ell_n \} }{\sigma}$}{
    $\varphi'_c \leftarrow $ \Rec{$\varphi_c$,$D$} \;
    \BlankLine

    \For{every $\ell$ in $\Conclusion{\varphi_c}$}{
      $\dl{\ell} \leftarrow$ the literal in $\Conclusion{\varphi'_c}$ corresponding to $\ell$, otherwise $\none$ \;
    }

    \Return{$\con{\varphi_c}{ \{\dl{\ell_1},\ldots,\dl{\ell_n} \} \backslash \{ \none \}  }{}$};
  }

  \caption[.]{\FuncSty{fo-delete}}
  \label{algo:fodel}
\end{algorithm}

The second challenge is harder to overcome. In the propositional case, collecting units and deleting units can be done in two distinct and independent phases (as in Algorithm \ref{algo:LU}). In the first-order case, on the other hand, these two phases seem to be so interlaced, that they appear to be in a deadlock: the decision to collect a unit to be lowered depends on what will happen with the proof after deletion, while deletion depends on knowing which units will be lowered.

A simple way of unlocking this apparent deadlock is depicted in Algorithm \ref{algo:FOLU}. It optimistically assumes that all units with more than one child are lowerable (lines 2-3). Then it deletes the units (line 6) and tries to reintroduce them in the bottom (lines 8-19). If the reintroduction of a unit $\varphi$ fails because the descendants of the literals that had been resolved with $\varphi$'s literal are not unifiable, then $\varphi$ is removed from the queue of collected units (lines 14-16) and the whole process is repeated, inside the \emph{while} loop (lines 5-19), now without $\varphi$ among the collected units. Since in the worst case the deletion algorithm may have to be executed once for every collected unit, and the number of collected units is in the worst case linear in the length of the proof, the overall runtime complexity is in the worst case quadratic with respect to the length of the proof. This is the price paid to disentangle the dependency between unit collection and deletion.

Alternatively, we could try to lower units incrementally, one at a time, always eagerly deleting the unit and reconstructing the proof immediately after it is collected. The optimistic approach of Algorithm \ref{algo:FOLU}, however, has the potential to save some deletion cycles.




\begin{algorithm}[bt]
  \SetAlgoVlined
  \SetAlgoShortEnd
  \KwIn {a proof $\psi$}
  \KwOut{a compressed proof $\psi^{\star}$}
  \KwData{a map $.'$: after line 4, it maps any $\varphi$ to \Del{$\varphi$, $D$}}
  \KwData{a map $\dl{.}$,mapping literals to changed literals,updated after every deletion}
  \BlankLine

  \SetKwData{Units}{Units}

  \SetKw{Remove} {remove}
  \SetKw{Break} {break}

  \algolines{\Units $\leftarrow \varnothing$}{queue to store collected units}
  \BlankLine

  \For{every subproof $\varphi$, in a bottom-up traversal of $\psi$}{
    \lIf{$\varphi$ is a unit with more than one child}{enqueue $\varphi$ in \Units}
  }
  \BlankLine

  \algolines{$s \leftarrow \texttt{false}$}{indicator of successful reintroduction of all units}

  \While{$\neg s$}{
    $\psi' \leftarrow $ \Del{$\psi$,$\Units$} \;
    \BlankLine

    \tcp{Reintroduce units}
    
    $s \leftarrow \texttt{true}$ \;

    $\psi^{\star} \leftarrow \psi'$ \;
    \For{every unit $\varphi$ in \Units}{
      \Let{$\{\ell\} = \Conclusion{\varphi}$} \;
      \Let{$\{ \ell_1, \ldots, \ell_n \}$ be the literals resolved against $\ell$ in $\psi$ } \;
      \Let{$c = \{ \dl{\ell_1},\ldots,\dl{\ell_n} \} \backslash \{ \none \}$} \;
      \Let{$c^{\downarrow}$ be the descendants of $c$'s literals in $\Conclusion{\psi'}$} \;
      \If{$c^{\downarrow}$'s literals are not unifiable}{
        $s \leftarrow \texttt{false}$ \;
        \Remove{$\varphi$ from \Units} \;
        \tcp{interrupt the for-loop}
        \Break \;
      }
      \ElseIf{$c^{\downarrow} \neq \emptyset$}{
        \Let{$\sigma$ be the unifier of $c^{\downarrow}$'s literals and $\ell^c$ the unified literal} \;
        $\psi^{\star} \leftarrow \con{\psi^{\star}}{c^{\downarrow}}{\sigma} \res{\ell^c}{}{\dl{\ell}}{} \varphi'$ \;
      }
    }
  }
    

  \caption{\FOLowerUnits}
  \label{algo:FOLU}
\end{algorithm}



==> sec-PropositionalAlgorithm.tex <==
\section{The Propositional Algorithm}

{\RPI} (formally defined in Appendix \ref{Section:RPI} and in \cite{LURPI}) removes \emph{irregularities}, which are resolution inferences deriving a node $\eta$ when the resolved literal occurs as the pivot of another inference located below in the path from $\eta$ to the root of the proof. In the worst case, regular resolution proofs can be exponentially bigger than irregular ones, but {\RPI} takes care of regularizing the proof only partially, removing inferences only when this does not enlarge the proof.

%ToDo: Informal textual description of the propositional algorithm, explaining what safe literals are. 
{\RPI} traverses the proof twice. On the first traversal (bottom-up), it computes and stores for each node a set of \emph{safe literals}: literals that are resolved in all paths from the node to the root of the proof or that occur in the root clause. If one of the node's resolved literals belongs to the set of safe literals, then it is possible to \emph{regularize} the node by replacing it by the parent containing the safe literal. To do this replacement efficiently, the replacement is postponed by marking the other parent as a \texttt{deletedNode}. Then, on a single second traversal (top-down), regularization is performed: any node that has a parent node marked as a \texttt{deletedNode} is replaced by its other parent.
%Refer reader to the CADE 2011 paper (where RPI is described) for a formal description of the propositional algorithm. 
% contains a formal description of {\RPI} (taken from \cite{LURPI}).
%Consider adding the formal description to an appendix in this paper, for the convenience of the reviewer.

The {\RPI} and the {\RP} algorithms differ from each other mainly in the
computation of the safe literals of a node that has many children. While the former 
returns the intersection as shown in Algorithm~\ref{algo:SetSafeLiterals}, the latter
returns the empty set. 
Moreover, while in {\RPI} the safe literals of the root node contain all the literals of the root clause, in {\RP} the root node is always assigned an empty set of literals. 

==> sec-PropositionalLU.tex <==

\section{The Propositional LowerUnits Algorithm}
\label{sec:PropositionalLU}

We denote by $\dn{\psi}{\varphi_1, \varphi_2}$ the result of deleting the subproofs $\varphi_1$ and $\varphi_2$ from the proof $\psi$ and fixing it according to Algorithm \ref{algo:del}\footnote{
  The deletion algorithm is a variant of the \textsc{Reconstruct-Proof} algorithm presented in \cite{RP11}.
  The basic idea is to traverse the proof in a top-down manner, replacing
  each subproof having one of its premises marked for deletion (i.e. in $D$) by its other premise (cf. \cite{Boudou}).
}. 
We say that a subproof $\varphi$ in a proof $\psi$ can be lowered 
if there exists a proof
$\psi'$ such that $\psi' = \dn{\psi}{\varphi} \odot \varphi$ and
$\Conclusion{\psi'} \subseteq \Conclusion{\psi}$. If $\varphi$ originally participated in many resolution inferences within $\psi$ (i.e. if $\varphi$ had many children in $\psi$) then lowering $\varphi$ compresses the proof (in number of resolution inferences), because $\dn{\psi}{\varphi} \odot \varphi$ contains a single resolution inference involving $\varphi$.

%
It has been noted in \cite{LURPI} that, in the propositional case, $\varphi$ can always be lowered if it is a \emph{unit} (i.e. its conclusion clause is unit). This led to the invention of {\LowerUnits} (Algorithm \ref{algo:LU}), which aims at transforming a proof $\psi$ into $(\dn{\psi}{\mu_1,\ldots,\mu_n}) \odot \mu_1 \odot \ldots \odot \mu_n$, where $\mu_1$, \ldots, $\mu_n$ are all units with more than one child. Units with only one child are ignored because no compression is gained by lowering them. The order in which the units are reintroduced is important:
if a unit $\varphi_2$ is a subproof of a unit
$\varphi_1$ then $\varphi_2$ has to be reintroduced later than (i.e. below) $\varphi_1$.


\newlength\algowd
\def\savewd#1{\setbox0=\hbox{#1\hspace{.7in}}\algowd=\wd0\relax#1}
\newcommand\algolines[2]{\savewd{#1}%
  \tcp*{\parbox[t]{\dimexpr\algowidth-\algowd}{#2}}}


\SetKwFunction{Del}{delete}
\SetKw{Let}{let}

\begin{algorithm}[bt]
  \SetAlgoVlined
  \SetAlgoShortEnd
  \KwIn{a proof $\varphi$}
  \KwIn{$D$ a set of subproofs}
  \KwOut{a proof $\varphi'$ obtained by deleting the subproofs in $D$ from $\varphi$}
  \KwData{a map $.'$, initially empty, eventually mapping any $\xi$ to \Del{$\xi$, $D$}}
  \BlankLine

  \newcommand{\fixL}{\ensuremath{\varphi'_L}}
  \newcommand{\fixR}{\ensuremath{\varphi'_R}}

  \lIf{$\varphi \in D$ or $\raiz{\varphi}$ has no premises}{\Return{$\varphi$}}
  \BlankLine

  \Else{
    \Let{$\varphi_L \res{\ell}{}{}{} \varphi_R = \varphi$} \;
    $\varphi'_L \leftarrow $ \Del{$\varphi_L$,$D$} \;
    $\varphi'_R \leftarrow $ \Del{$\varphi_R$,$D$} \;
    \BlankLine

    \lIf{$\varphi'_L \in D$}{ \Return{\fixR} }
    \lElseIf{$\varphi'_R \in D$}{ \Return{\fixL} }
    \BlankLine

    \lElseIf{$\ell \notin \Conclusion{\fixL}$}{ \Return{\fixL} }
    \lElseIf{$\dual{\ell} \notin \Conclusion{\fixR}$}{ \Return{\fixR} }
    \BlankLine

    \lElse{ \Return{ \fixL~$\res{\ell}{}{}{}$~\fixR} }
  }

  \caption[.]{\FuncSty{delete}}
  \label{algo:del}
\end{algorithm}



\begin{algorithm}[bt]
  \SetAlgoVlined
  \SetAlgoShortEnd
  \KwIn {a proof $\psi$}
  \KwOut{a compressed proof $\psi^{\star}$}
  \KwData{a map $.'$: after line 4, it maps any $\varphi$ to \Del{$\varphi$, $D$}}
  \BlankLine

  \SetKwData{Units}{Units}
  \algolines{\Units $\leftarrow \varnothing$}{queue to store collected units}
  \BlankLine

  \For{every subproof $\varphi$, in a bottom-up traversal of $\psi$}{
    \lIf{$\varphi$ is a unit with more than one child}{enqueue $\varphi$ in \Units}
  }
  \BlankLine

  $\psi' \leftarrow $ \Del{$\psi$,$\Units$} \;
  \BlankLine

  \tcp{Reintroduce units}
  $\psi^{\star} \leftarrow \psi'$ \;
  \For{every unit $\varphi$ in \Units}{
    \Let{$\{\ell\} = \Conclusion{\varphi}$} \;
    \lIf{$\dual{\ell} \in \Conclusion{\psi'}$}{
    $\psi^{\star} \leftarrow \psi^{\star} \odot_\ell \varphi'$}
  }

  \caption{\LowerUnits}
  \label{algo:LU}
\end{algorithm}

In Algorithm \ref{algo:LU}, units are collected in a queue
during a bottom-up traversal (lines 2-3), then they are deleted from the proof (line 4) and finally reintroduced in the bottom of the proof (lines 5-7). In \cite{Boudou} it has been observed that the two traversals (one for collection and one for deletion) could be merged into a single traversal, if we collect units during deletion. As deletion is a top-down traversal, it is then necesary to collect the units in a stack. This improvement leads to Algorithm \ref{algo:optLU}. Both algorithms have a linear run-time complexity with respect to the length of the proof, because they perform a contant number of traversals.


\begin{algorithm}[pbt]
  \SetAlgoVlined
  \SetAlgoShortEnd
  \SetKwData{Units}{Units}

  \KwIn {a proof $\psi$}
  \KwOut {a compressed proof $\psi^{\star}$}
  \KwData{a map $.'$, eventually mapping any $\varphi$ to \Del{$\varphi$, \Units}}
  \BlankLine

  \SetKw{Push}{push}
  \SetKw{Pop} {pop}
  \SetKw{Add} {add}
  \SetKw{Rep} {replace}

  \algolines{$D \leftarrow \varnothing$}{set for storing subproofs that need to be deleted}
  \algolines{\Units $\leftarrow \varnothing$}{stack for storing collected units}
  \BlankLine

  \For{every subproof $\varphi$, in a top-down traversal of $\psi$ }{

    \lIf{$\varphi$ is an axiom}{$\varphi' \leftarrow \varphi$}
    \Else{
      \Let{$\varphi_L \odot_{\ell} \varphi_R = \varphi$} \;
      \lIf{ $\varphi_L \in D$ and $\varphi_R \in D$}{
        \Add $\varphi$ to $D$
      }
      \lElseIf{$\varphi_L \in D$}{
          $\varphi' \leftarrow \varphi'_R$
      }
      \lElseIf{ $\varphi_R \in D$ }{
          $\varphi' \leftarrow \varphi'_L$
      }

      \BlankLine

      \lElseIf{$\ell \notin \Conclusion{\varphi'_L}$}{ $\varphi' \leftarrow \varphi'_L$ }
      \lElseIf{$\dual{\ell} \notin \Conclusion{\varphi'_R}$}{ $\varphi' \leftarrow \varphi'_R$  }
    
      \lElse{ $\varphi' \leftarrow \varphi'_L \odot_{\ell} \varphi'_R$ }

        
    }
    \BlankLine
  
    \If{$\varphi$ is a unit with more than one child}{
      \Push $\varphi'$ onto \Units  \;
      \Add $\varphi$ to $D$ \;
    }
  }
  \BlankLine


  \tcp{Reintroduce units}
  $\psi^{\star} \leftarrow \psi'$ \;
  \While{\Units $\neq \varnothing$}{
    $\varphi' \leftarrow$ \Pop from \Units \;
    \Let{$\{\dual{\ell}\} = \Conclusion{\varphi}$ } \;
    \lIf{$\ell \in \Conclusion{\psi^{\star}}$ \label{line:full:testreintroduce}  }{
      $\psi^{\star} \leftarrow \psi^{\star} \odot_{\ell} \varphi'$ }
  }

  \caption{Improved {\LowerUnits} (with a single traversal)}
  \label{algo:optLU}
\end{algorithm}




==> sec-SimpleFOLU.tex <==

\section{A Linear Greedy Variant of First-Order LowerUnits}
\label{sec:SimpleFOLU}

The {\FOLowerUnits} described in the previous section is not only complex (worst-case quadratic run-time complexity in the length of the input proof) but also difficult to implement. The necessity to ensure the post-deletion unifiability property would require a lot of bookkeeping, to track changes in literals and their descendants, and to know which literals have to be contracted in the bottom of the proof before reintroduction of the units. 

This section presents {\SFOLowerUnits} (Algorithm \ref{algo:optSFOLU}), an alterantive (single traversal) variant of {\FOLowerUnits}, which avoids the quadratic complexity and the implementation difficulties by: 1) ignoring the stricter post-deletion unifiability property and focusing instead on the pre-deletion unifiability property, which is easier to check (lines 9-11); and 2) employing a greedy contraction approach (lines 16-18) together with substitutions (lines 5-7), in order not to care about bookkeeping. By doing so, compression may not always succeed on all proofs (e.g. Example \ref{ex:rootpair}). When compression succeeds, the root clause of the generated proof will be the empty clause (line 20) and the generated proof may be returned. Otherwise, the original proof must be returned (line 20).


\begin{algorithm}[pbt]
  \SetAlgoVlined
  \SetAlgoShortEnd
  \SetKwData{Units}{Units}

  \KwIn {a proof $\psi$}
  \KwOut {a compressed proof $\psi^{\star}$}
  \KwData{a map $.'$, eventually mapping any $\varphi$ to \Del{$\varphi$, \Units}}
  \BlankLine

  \SetKw{Push}{push}
  \SetKw{Pop} {pop}
  \SetKw{Add} {add}
  \SetKw{Rep} {replace}

  \algolines{$D \leftarrow \varnothing$}{set for storing subproofs that need to be deleted}
  \algolines{\Units $\leftarrow \varnothing$}{stack for storing collected units}
  \BlankLine

  \For{every subproof $\varphi$, in a top-down traversal of $\psi$ }{

    \lIf{$\varphi$ is an axiom}{$\varphi' \leftarrow \varphi$}
    \ElseIf{$\varphi = \varphi_L \res{\ell_L}{\sigma_L}{\ell_R}{\sigma_R} \varphi_R$}{
      \lIf{ $\varphi_L \in D$ and $\varphi_R \in D$}{
        \Add $\varphi$ to $D$
      }
      \lElseIf{$\varphi_L \in D$}{
          $\varphi' \leftarrow \con{\varphi'_R}{}{\sigma_R}$
      }
      \lElseIf{ $\varphi_R \in D$ }{
          $\varphi' \leftarrow \con{\varphi'_L}{}{\sigma_L}$
      }

      \BlankLine

      \lElseIf{$\ell \notin \Conclusion{\varphi'_L}$}{ 
        $\varphi' \leftarrow \con{\varphi'_L}{}{\sigma_L}$ 
      }
      \lElseIf{$\dual{\ell} \notin \Conclusion{\varphi'_R}$}{ 
        $\varphi' \leftarrow \con{\varphi'_R}{}{\sigma_R}$  
      }
    
      \lElse{ $\varphi' \leftarrow \varphi'_L \res{\ell_L}{\sigma_L}{\ell_R}{\sigma_R} \varphi'_R$ }

        
    }
    \lElseIf{$\varphi = \con{\varphi_c}{ \{\ell_1,\ldots,\ell_n \} }{\sigma}$}{
      $\varphi' \leftarrow \con{\varphi'_c}{ \{\ell_1,\ldots,\ell_n \} }{\sigma}$
    }

    \BlankLine
  
    \If{$\varphi$ is a unit with more than one child satisfying the pre-deletion unifiability property}{
      \Push $\varphi'$ onto \Units  \;
      \Add $\varphi$ to $D$ \;
    }
  }
  \BlankLine


  \tcp{Reintroduce units}
  $\psi^{\star} \leftarrow \psi'$ \;
  \While{\Units $\neq \varnothing$}{
    $\varphi' \leftarrow$ \Pop from \Units \;

    $\psi^{\star}_{\mathrm{next}} \leftarrow \con{\psi^{\star}}{}{}$ \;
    \While{$\Conclusion{\psi^{\star}_{\mathrm{next}}} \neq \psi^{\star} $}{
      $\psi^{\star} \leftarrow \psi^{\star}_{\mathrm{next}}$ \;
      $\psi^{\star}_{\mathrm{next}} \leftarrow \con{\psi^{\star}}{}{}$ \;
    }

    
    \lIf{$\psi^{\star} \odot \varphi'$ is well-defined}{
      $\psi^{\star} \leftarrow \psi^{\star} \odot \varphi'$ }

  }

  \lIf{$\Conclusion{\psi^{\star}} = \bot$}{\Return{$\psi^{\star}$}}
  \lElse{\Return{$\psi$}}

  \caption{{\SFOLowerUnits} (single traversal)}
  \label{algo:optSFOLU}
\end{algorithm}



% \begin{algorithm}[bt]
%   \SetAlgoVlined
%   \SetAlgoShortEnd
%   \KwIn {a proof $\psi$}
%   \KwOut{a compressed proof $\psi^{\star}$}
%   \KwData{a map $.'$: after line 4, it maps any $\varphi$ to \Del{$\varphi$, $D$}}
%   \BlankLine

%   \SetKwData{Units}{Units}

%   \SetKw{Remove} {remove}
%   \SetKw{Break} {break}

%   \algolines{\Units $\leftarrow \varnothing$}{queue to store collected units}
%   \BlankLine

%   \For{every subproof $\varphi$, in a bottom-up traversal of $\psi$}{
%     \lIf{$\varphi$ is a unit with more than one child and all literals of $\varphi$ are simultaneously unifiable}{enqueue $\varphi$ in \Units}
%   }
%   \BlankLine

%     $\psi' \leftarrow $ \FuncSty{simple-fo-delete}$(\psi,\Units)$ \;
%     \BlankLine

%     \tcp{Reintroduce units}
    

%     $\psi^{\star} \leftarrow \psi'$ \;
%     \For{every unit $\varphi$ in \Units}{
%         \Let{$\sigma$ be the unifier of $\rho(\psi^\star)$'s literals that contracts $\rho(\psi^\star)$ as much as possible} \;
%         \Let{$c$ be the literals contracted by $\sigma$} \;
%        \If{$ \con{\psi^{\star}}{c}{\sigma}$ and $\varphi$ can be resolved} {
%         $\psi^{\star} \leftarrow \con{\psi^{\star}}{c}{\sigma} \res{\ell^c}{}{\ell}{} \varphi$ \;
%         }\Else { \Return $\psi$}
      
%     }
  
    

%   \caption{\SFOLowerUnits}
%   \label{algo:simpleFOLU}
% \end{algorithm}

% Algorithm \ref{algo:simpleFOLU} works similarly to the propositional algorithm.  It first performs a bottom up traversal to collect units which satisfy Property \ref{prop:pair}, adding those that do to a queue (line 3). It then attempts to re-introduce all the removed units at the bottom of the proof, where it attempts to compress the literals that would be resolved away by each unit (lines 6-15). In order to avoid traversing the proof to find literals resolved away from by each unit again after the deletion of every potential unit (as is done in Algorithm \ref{algo:FOLU}), we use a modified \FuncSty{delete} function, called \FuncSty{simple-fo-delete}, which is the same as Algorithm \ref{algo:del} except with line 6 changed to the following:

%    \lIf{$~\varphi'_L \in D~$}{ 
%      \Return{$(\rho(\varphi'_L) \sigma_R)$} 
%     }
%     \lElseIf{$\varphi'_R \in D$}{ 
%       \Return{$(\rho(\varphi'_R) \sigma_R)$}  
%     }

% \FuncSty{simple-fo-delete} is designed to reduce the complexity of tracking literals. \FuncSty{simple-fo-delete} behaves much more closely to the propositional case and requires none of the additional data structures required by \FuncSty{fo-delete}. In this function, when a unit node is deleted, instead of returning the opposite node (respectively $\psi_L'$ or $\psi_R'$, line 6) in the resolution (which is done in the propositional case), or tracking the literals (which is done in \FuncSty{fo-delete}), we return the opposite node with $\sigma_L$ (respectively $\sigma_R$) applied to its root clause. In this way, the literals not resolved with the unit will look like they would have in the original proof, and the literals which were not resolved due to the deletion looks like it is syntactically equal with the unit literal at this stage. The fact that the other literals look like they did in the original proof is key: now resolution in the compressed proof can use the old literals, which should appear as they before, and not worry about choosing the wrong literal in case of ambiguous resolution. 

% %A negative side-effect of this is that we may end up grounding literals, and having to carry these forms of each literal forward, which may increase the character length of the clause, though not the number of nodes in the proof.

% However, we can not guarantee that Property \ref{prop:rootpair} is satisfied. The appearance of literals that were to be resolved away from a unit clause may have changed, preventing completion of the proof. If this happens {\SFOLowerUnits} will attempt to re-introduce this node and fail, returning the original input proof (line 12). As a result, some proofs that can be compressed are returned unmodified, but those that do not require this additional property can be compressed much more quickly.

% Alternatively, if additional unifiers do not modify the literals resolved away by a unit, those literals will still satisfy Property \ref{prop:pair}, and any contraction that reduces the length by as much as possible, such as one found in line 7, will reduce these literals to a single literal, which will be unifiable with the unit. 



%\input{simple-fo-delete-full}




==> simple-fo-delete-full.tex <==
\begin{algorithm}[bt]
  \SetAlgoVlined
  \SetAlgoShortEnd
  \KwIn{a proof $\varphi$}
  \KwIn{$D$ a set of subproofs}
  \KwOut{a proof $\varphi'$ obtained by deleting the subproofs in $D$ from $\varphi$}
  \BlankLine

  \newcommand{\fixL}{\ensuremath{\varphi'_L}}
  \newcommand{\fixR}{\ensuremath{\varphi'_R}}

  \lIf{$\varphi \in D$ or $\raiz{\varphi}$ has no premises}{\Return{$\varphi$}}
  \BlankLine

  \Else{$\varphi = \varphi_L \res{\ell_L}{\sigma_L}{\ell_R}{\sigma_R} \varphi_R$\;
    $\varphi'_L \leftarrow $ \Rec{$\varphi_L$,$D$} \;
    $\varphi'_R \leftarrow $ \Rec{$\varphi_R$,$D$} \;
    \BlankLine

    \lIf{$\varphi'_L \in D$}{ 
      \Return{$($\fixR $\sigma_R)$} 
    }
    \lElseIf{$\varphi'_R \in D$}{ 
      \Return{$($\fixL $\sigma_R)$}  
    }
    \BlankLine


    \lElse{ 
      \Return{ \fixL~$\res{\ell_L}{}{\ell_R}{}$~\fixR}
    }
  }



  \caption[.]{\FuncSty{simple-fo-delete}}
  \label{algo:sfodel}
\end{algorithm}
